Learning to Ask Informative Questions: Enhancing LLMs with Preference Optimization and Expected Information Gain

Questions are essential tools for acquiring the necessary information to complete information-seeking tasks. However, large language models (LLMs), especially open-source models, often perform poorly in generating informative questions, as measured by expected information gain (EIG). In this paper, we propose a method to enhance the informativeness of LLM-generated questions in 20-question game dialogues. We sample multiple questions from the same model (LLAMA 2-CHAT 7B) for each game and create pairs of low-EIG and high-EIG questions to apply a Direct Preference Optimization (DPO) algorithm. Our results show that this method produces more effective questions (in terms of EIG), even in domains different from those used to train the DPO model.

==> latex/experiments.tex <==

\section{Experiments}

\subsection{Applications and Datasets}
20 Questions Game

Medical Diagnosis

20 Questions Game: INLG, Apple, BigBench, Common (?)

Medical Diagnosis: (?)

%\subsection{Baselines} What is the answerer? Same model or GPT-4 (+ more fair) ma il nostro modello svantaggiato? Llama-13B, Llama-70B (4 bit == 35GB ram == 2 GPUs from clic4). Llama-13B and 70B with CoT and UoT

\subsection{Evaluation Metrics}

\emph{game} and \emph{dialogue}

\tb{insert new metrics}

Questions' informativeness is measured through Mean conversation Length in Successful cases (MLS), Success Rate (SR), Mean Conversation Length (ML). Mean Conversation Length in Successful Cases measures the number of questions required to achieve the target in successful cases only. Since each game is repeated until it meets the successful condition once, the number of successful games is equal to the number of candidates set. The Success Rate measures how many times the model achieve the target at the first try (e.g., without repetition). Mean Conversation Length takes into consideration unsuccessful tries required to achieve the target, each unsuccessful equal to 20 questions. 


==> latex/old_introduction.tex <==
\section{Introduction}
\label{sec:intro}

%LLMs + surveys on benchmarks and reasoning
%Conversational Seeking Dialogues
%LINK: problem solver
%DECOMPOSE COMPLEX PROBLEMS
%QUESTION GENERATION
%Decompose coplex problems into smaller ones

%Now that the AI community has at its disposal models that master language well, the next challenge is to equip them with the ability to seek information to solve a problem. Being able to ask informative questions is a key ingredient to being a good problem solver. One of the easiest settings for such an information-seeking challenge is the \emph{20 Questions Game}, traditionally used in Cognitive studies to study human intelligence (e.g.~\citet{mosh:onas66,RUGGERI2015203}), and now under the lens of AI researchers (e.g.~\citet{}). 

%QUESTIONS
Questions in language are request for information \citep{Hiz1978Questions}. The speaker lacks information in his knowledge state, and ask a question to elicit this. Solving complex problems often requires this process of eliciting information through questions, as not all the required information are explicit in the problem statement \citep{Geva2021Aristotle}. Consider, for instance, a medical interview: the doctor makes questions to elicit the patient's sign and symptoms. Once enough information has been collected, the doctor identify the disease and proceed with a treatment. 
% Linguistic definition of a question: "an utterance that 'craves' a verbal response".

%Cognitive Science Studies: 20 Questions Game, EIG and results on Humans
Not all questions, however, are equally informative. Some questions are more efficient to reach the problem's solution than others. To study questions' informativeness, two interesting tools emerge from Cognitive Science  \citep{RUGGERI2015203}: the 20 Questions Game as a test bed, and the Expected Information Gain as a quantifying measure. The \emph{20 Questions game} consists of one player asking yes/no questions to identify the item the other player has in mind, from a pool of possible items. In this context, the \emph{Expected Information Gain} \citep{} measures questions' informativeness as the reduction in entropy caused by a certain question in the space of possible items. Most informative questions are the ones partitioning the possible items in two equal clusters, expecting a positive answer for half of them and a negative for the remaining half. Humans have been shown to ask informative questions when the number of possible items is limited \citep{}, yet struggling when many candidates are available (due to limited working memory).
%LINK: TYPES OF QUESTIONS IN THE 20Q GAME
%LINK: 'request for information' --> informative questions

%OR 
%Humans and Pratical applications
%Humans tend to ask informative yes/no questions when the number of possible items is limited \citep{}. Due to the limited working memory, however, they struggle asking informative questions when many items are available \citep{}. Considering all the . And this is even more difficult in real open settings, where the possible candidates are not explicit at the beginning. The underlying ability of solving this game is bounded to real-world problems. 
%LLMs and Related Works

%LLMs limitation, Human limitation, practical applications
Large Language Models (LLMs) have shown increasing language and reasoning capabilities \citep{}. Due to the massive knowledge encoded in their parameters, LLMs' may be able to identify relational features linking items together. This make, in theory, LLMs able to cluster several items in different configurations and asking informative questions in setting where humans are limited. Despite this intuition, LLMs seems to struggle to generate informative questions and solve the 20 Questions Game \citep{Apple}. As a result of their training and optimisation process, LLMs generate correct and reasonable questions, but characterized by low informativeness \citep{INLG23}. How to make LLMs more informative questioner is the main purpose of our study.

%CFR. with humans (anche peggio degli umani!)
%Why LLMs do bad
%Why LLMs could do better than humans
%Practical Applications

%\tb{Say why the game is important.. broader.. Uncertanity? Clarification question? Or be of help in contexts when the candidates are many and humans have difficulty?}

%Current methods: super-relevant related work & Our contribution 
%What is the gap in the literature that we address? What do we do better?

%RB

%our research Questions

%RBThe aim of this study is to improve open-source LLMs to ask more informative questions. 
As illustrated in Figure~\ref{fig:bootstrapping}, our proposed method comprises three steps: questions generation, questions evaluation in terms of EIG, preference optimization (RL). All these steps are accomplished by the same open-source model, without relying on data from external models. In the first step, the model generates some possible questions, then it computes the relative EIG for each question. This collections of informative and less informative questions are used for RL with Direct Preference Optimization (DPO; \citealt{rafailov2024direct}). We observe that LLMs can learn to ask more informative questions, but does this ability generalize to unseen scenarios? And finally, does this ability generalize to different applications?

%RIASSUNTO HU: The model generates a series of questions and their possible follow-up questions, selecting the question leading to higher expected information gain overall. 

%In Cognitive Science, the \emph{20 Questions Game} has been traditionally employed to investigate the developing abilities of children in searching for information.  

%OPEN VS CLOSED SETTING
%In this two-player game, one player makes yes/no questions to identify the candidate the other player has in mind.  Questions pointing to features shared among candidates are more informative than tentative solutions. The game can be played either by providing the set of possible candidates/hypotheses (closed version) or by leaving the hypothesis space open (open version). In the former case, the questioner has to put at work two main skills: reasoning about informativeness and reasoning incrementally and coherently as new information is obtained; while, in the open setting only the second skill is tested.
%LINK: Linguistic ony yes/no questions, a degenerate case of XXX question

\begin{figure}
\includegraphics[]{images/Bootstrapping.png}
\end{figure}

%In the close version, given a set of candidates, one player makes yes/no questions to identify the candidate the other player has in mind. Questions pointing to features shared among candidates are more informative than tentative solutions. 

%CAPACITà COINVOLTE
%Sono coinvolte due capacità diverse: ragionare in termini di informatività e procedere in maniera coerente e consequenziale rispetto alle domande precedenti. Nel closed setting sono coinvolte entrambe le capacità, in quello open solo la seconda. Il nostro bootstrapping con max EIG e stepwise, garantisce entrambe.

%più approfondito
%RB I removed the part below. 
%Through qualitative measures and expected information gain (EIG), cognitive studies observed a developmental shift of children from low- to high-informative questions. Our work delves into the information-seeking strategy of large language models (LLMs), focusing on the shift across LLMs of different sizes and strategies to improve their performances. \rb{WE HAVE TO MAKE OUR GOAL clearer.}

% Our setting tests LLMs with hierarchical candidate spaces, comparing LLMs with humans and an optimal agent (for EIG). We observe that a big LLM (ChatGPT) is closer to humans and the optimal agent than a smaller one (Llama-2).

%Both LLMs improve their strategy when prompted to reason stepwise, while struggle with negative answers. Our current focus is on improving Llama-2 questions’ informativeness with supervised fine-tuning (SFT) and reinforcement learning (RL). SFT requires annotated data, collected with bootstrapping: the model has been playing as both players, saving only questions maximizing EIG (10.000 dialogues). RL, instead, employs EIG as an automatically computed reward function, giving the model the ability to distinguish between high and low informative questions. Along with overall improvements, we will analyse the impact of both methods in processing negation.


==> latex/old_related_work.tex <==

\section{Related Works}

\tb{espite the implications in real-world scenarios, such as Medical Diagnosis and Conversational Search, the task of Question Generation is understudied in the Computational Linguistics community \citep{}. Some researchers have recently pointed the attention to this task, working to improve open-source LLMs' in the 20 Questions Game. After evaluating recent LLMs, \citealp{Apple} improves open-source LLMs via Reinforcement Learning (RL). Their implementation of RL relies on a raw reward function, directly optimising the model to achieve the target with fewer questions. Without training models, \citealp{hu:unce24} propose a re-ranking strategy based on Expected Information Gain of questions and foreseen follow-up questions. To train a model to reason about informativeness, we propose a training strategy leveraging Expected Information Gain as a refined reward function in a RL loop. 
}

%Question asking is central to human learning, hence, information-seeking games have been largely used in the cognitive science literature to study the developmental trajectory of humans (see e.g.,~\citealt{mosh:onas66,RUGGERI2015203}). 

In the computational literature in the past, attention has been put on the need to enhance models with the ability to ask questions that maximize the expected information gain from a possible answer (eg.~\cite{NIPS2017_24681928,rao-daume-iii-2018-learning}).  The Twenty Questions game, though simple in its settings, has been proposed to evaluate models' information-seeking skills~\citet{srivastava2023beyond,INLG23,hu:unce24} \rb{results?}. Following the cognitive science literature~\cite{Ruggeri21HowTo}, \citet{INLG23} use a hierarchically organized hypothesis space and show that prompting the model to explicitly update the hypothesis space at each turn increases GPT-3.5 performance, yet results are still far away from those of an optimal model. 
%This game is usually framed as a dialogue between two participants: one of them is secretly assigned an entity (i.e., a target) and the other has to guess it by asking a series of questions. The set of objects that can be possible targets is defined as the `hypothesis space'. Depending on the experimental setup, the hypothesis space can be defined a priori (making the game easier) or not. Even in a closed hypothesis space setting (viz., with listed candidates), 
Today proprietary large language models, such us PaLM70B~\cite{anil2023palm} or GPT-4~\cite{}, still reach low task accuracy~\cite{hu:unce24}. 

To overcome such limitation, a first approach is to let the model generate several questions and then re-rank them based on either the probability distribution change in the hypothesis space~\cite{Confirm-it} or on a verification step computing the expected information gain~\cite{grand:LIPS,hu:unce24}. Among this work, \cite{hu:unce24} is the closest to us. \dm{describe and say what is the limitation} %rao-daume-iii-2018-learning rerank based on how useful is the answer.

An alternative approach lets models go under a supervised fine-tuning step, and iteratively train models on self-generated data~\cite{suglia-etal-2021-empirical,testoni:garb22} or data generated by a bigger model~\cite{Apple}.
%. and such iteration proved beneficial to let the model avoid deteriorating their behavior at inference time when encountering a mistake. 
Following up and extending the bootstrapping approach based on a self-improvement loop proposed in~\citet{STAR22}, \cite{andukuri2024stargate} teaches a small-size language model, Mistral7B, to ask clarifying questions for eliciting user preferences. The model is iteratively fine-tuned on self-produced high-quality questions, namely questions that elicit high-quality responses. Similarly to this work, our method starts with a bootstrapping self-improved loop to collect high-quality questions that we select based on their Expected Information gain (EIG). We use a preference optimization algorithm, DPO~\cite{rafailov2024direct}, to teach the model to ask follow-up questions with high EIG given the previous context and the set of candidates. \at{I feel like we should clarify the novelty of the approach here.}

In the past, RL has been used in a variety of information-seeking settings \cite{stru:end17,shukla-etal-2019-ask,qi-etal-2020-stay}.  The use of DPO lets us overcome the computational costs of a standard Reinforcement Learning approach (RL). \dm{explain}. 

%\at{I think the remaining part of the paragraph can be drastically shortened.} RL has been proposed in information-seeking tasks in several forms and domains. For instance, \cite{stru:end17,shukla-etal-2019-ask} applied it in a visually grounded context to identify a target among a set of objects, a closed hypothesis space, while\citey{qi-etal-2020-stay} exploited RL to tackle the rather challenging scenario of open space information-seeking conversation. More recently,\citet{pyatkin-etal-2023-clarifydelphi} used it in social and moral situations to teach the model to ask defeasible clarification questions; and inspired by the recent success of RL based on Human Feedback,\citet{Apple} propose RL from Game-play (RLGP).\dm{explain plus say Our work is similar to \citet{Apple} but xxx} 

\dm{In sum, We combine these approaches. Using EIG as metric for the direct optimization of informative self-generated questions.}

%In Cognitive Science, the 20 Questions Game has been employed to study the developmental trajectory of question answer generation \citealt{}.  BOTH WITH IMAGES AND ONLY WORDS. ------- CLOSED VERSION ---------
%At the intersection of Cognitive Science and Computational Linguistics, \citealt{Testoni23} introduce the EXPECTED INFORMATION GAIN (EIG) [...] 


\cut{In Computational Linguistics, the 20 Questions Game has been recently employed by \citealt{INLG23} to test ChatGPT questions' informativeness. In a language-only and closed version of the game, the authors propose two ChatGPT's instances playing the roles of the questioner and the answerer. Measuring both EIG and the average numbers of turns to solve the game with hierarchical candidates' spaces, ChatGPT performances have been observed to be suboptimal and even worse than a random guessing strategy. \citealt{Apple} propose a systematic study on several LLMs with the open version of the game. Interestingly, the authors help open-source LLMs solving the game in fewer turns through a straightforward Reinforcement Learning reward. 
Multi-turn guessing games have been studies in multi-modal settings. GuessWhat?! and GuessWho?
The GuessWhat?! dataset is one of the most interesting, where the agent should [...]
To achieve better performances on the GuessWhat?! dataset \citealp{}, \citealt{Confirm-it} propose a re-ranking strategy to guide a XXX model. 
\citealt{Jorge2017learning} frames GuessWho? with images as a multi-agent reinforcement learning game. The model learn to play both roles, leveraging words grounded in the images and using information from previous steps. Finally, \citealt{GroundedRetrieval23} [...]
}

==> latex/related_work.tex <==
\section{Related Work}

%Despite the implications in real-world scenarios, such as Medical Diagnosis and Conversational Search, the task of Question Generation is understudied in the Computational Linguistics community \citep{}. 
The two recent work closest to us are \citet{Apple} and \citet{hu:unce24}
\citealp{Apple} improves open-source LLMs via Reinforcement Learning (RL). Their implementation of RL relies on a raw reward function, directly optimizing the model to achieve the target with fewer questions. Without training models, \citealp{hu:unce24} propose a re-ranking strategy based on EIG of questions and foreseen follow-up questions. Differently from them, we propose a training strategy leveraging EIG as a refined reward with direct preference optimization. \dm{advantage?} 
